Learning Joint Synchronization, Channel Estimation, and Decoding: Comparison with a Finite-Blocklength Achievability Bound

Learned schemes that jointly perform tasks such as synchronization and decoding have achieved promising results for short-packet communication. However, it remains unclear how close their performance is to information-theoretic bounds. To investigate this question, we extend the turbo autoencoder (TurboAE) proposed in D\"orner et al. (2023) to a single-input single-output waveform channel with an unknown delay and memoryless block fading, for which an achievability bound from finite-blocklength information theory is available. Our extension incorporates a pilot-free, model-guided neural synchronizer and enables joint synchronization, channel estimation, and decoding. At a blocklength of $64$ complex symbols and a rate of one bit per channel use, the proposed TurboAE achieves a lower bit error rate (BER) than all evaluated pilot-assisted 5G baselines, with gains of $1.9$ dB at a BER of $10^{-3}$ over a baseline involving a low-density parity-check (LDPC) code and $1.7$ dB over a baseline involving a polar code and successive cancellation list decoding (list size $8$). In terms of block error rate (BLER), the TurboAE outperforms the LDPC-coded baseline, but lags behind the polar-coded baseline by about $0.8$ dB at a BLER of $10^{-3}$. Moreover, all evaluated schemes remain at least $2.1$ dB away from a pilot-assisted achievability bound, indicating substantial room for improved designs.

==> diagrams/tikz/system_model_2.tex <==
\includegraphics{diagrams/system_model_2.png}

==> diagrams/tikz_src/Readme.tex <==
% use the following command to convert .tex file to .pdf file when submitting the paper

% pdflatex -interaction=nonstopmode -halt-on-error -jobname=example -output-directory=diagrams/tikz '\documentclass[tikz,border=2pt]{standalone}\usepackage{xcolor}\usepackage{pgfplots}\pgfplotsset{compat=1.18}\input{preambles/colors.tex}\begin{document}\input{diagrams/tikz/example.tex}\end{document}'

==> diagrams/tikz_src/conventional_baseline.tex <==
% Asymmetric cloud path adapted from https://tex.stackexchange.com/questions/45404/asymmetric-cloud-shape-in-tikz
% Original by Alain Matthes
\providecommand{\conventionalbaselineasymcloud}[2][0.2]{%
    \begin{scope}[#2]
        \pgftransformscale{#1}%
        \pgfpathmoveto{\pgfpoint{261 pt}{115 pt}}
        \pgfpathcurveto{\pgfqpoint{70 pt}{107 pt}}
                       {\pgfqpoint{137 pt}{291 pt}}
                       {\pgfqpoint{260 pt}{273 pt}}
        \pgfpathcurveto{\pgfqpoint{78 pt}{382 pt}}
                       {\pgfqpoint{381 pt}{445 pt}}
                       {\pgfqpoint{412 pt}{410 pt}}
        \pgfpathcurveto{\pgfqpoint{577 pt}{587 pt}}
                       {\pgfqpoint{698 pt}{488 pt}}
                       {\pgfqpoint{685 pt}{366 pt}}
        \pgfpathcurveto{\pgfqpoint{840 pt}{192 pt}}
                       {\pgfqpoint{610 pt}{157 pt}}
                       {\pgfqpoint{610 pt}{157 pt}}
        \pgfpathcurveto{\pgfqpoint{531 pt}{39 pt}}
                       {\pgfqpoint{298 pt}{51 pt}}
                       {\pgfqpoint{261 pt}{115 pt}}
        \pgfusepath{fill,stroke}%
    \end{scope}%
}

\begin{tikzpicture}[
    % Fit an IEEE column through native geometry rather than scaling the
    % complete picture, so the figure text remains at caption size.
    x=1cm,
    y=1cm,
    font=\footnotesize,
    >=latex,
    block/.style={
        draw=black,
        rounded corners=1pt,
        minimum width=1.00cm,
        minimum height=0.8cm,
        align=center,
        text width=1.30cm,
        inner sep=0.5pt
    },
    dashedbox/.style={
        rounded corners=1.0pt,
        line width=.65pt,
        align=center,
        inner sep=2pt
    },
    module/.style={
        rounded corners=3.0pt,
        line width=.65pt,
        align=center,
        inner sep=2pt
    },
    signal/.style={
        ->,
        line width=0.55pt
    }
]
    % \node at (0,0) {x};
    % \node at (1,0) {x};
    % \node at (0,1) {x};
    % \node at (1,1) {x};

    % \draw[dashedbox, draw=mittelblau, fill=mittelblau]
    %     (-0.80,0.92) rectangle (4.0,2.70);
    % \node at (3.35,2.50) {Encoder};

    % \draw[dashedbox, draw=orange!70!black, fill=orange!70!black]
    %     (-0.80,-1.00) rectangle (4.0,0.8);
    % \node at (3.35,-0.8) {Decoder};

    \node[module,draw=e2eGold,fill=e2eGoldFill,
      minimum width=3.25cm,minimum height=2.40cm] (channel_box) at (5.7,0.67) {};


    \node[] at (-0.95,1.0){$\vecu$};
    \node[] at (-0.95,-0.3){$\hat{\vecu}$};
    \node[] at (3.9,1.0){$\vecx$};
    \node[] at (3.9,-0.3){$\vecy$};



    \node[block] (enc) at (-0.05,1.3) {Channel\\Encoder};
    \node[block] (map) at (1.55,1.3) {Symbol\\Mapper};
    \node[block] (pilot) at (3.10,1.3) {Pilot\\Insertion};
    \node[block] (pulse) at (4.95,1.3) {Pulse\\Shaping};
    \node[inner sep=0pt, outer sep=0pt] (chan) at (6.55,1.3)
        {\tikz{\conventionalbaselineasymcloud[0.07]{fill=platinum, line width=0.55pt}}};
    \node[align=center, yshift=-2pt] at (chan)
        {Delay\\[1pt]Fading};
    \node[block] (dec) at (-0.05,0.00) {Channel\\Decoder};
    \node[block] (CSI) at (1.55,0.00) {CSI\\Est.};
    \node[block] (sync) at (3.10,0.00) {Sync.};
    \node[block] (oversampling) at (4.95,0.00) {Over-\\sampling};
    \node[block] (filter) at (6.55,0.00) {Filtering};


    \draw[signal] ([xshift=-10pt]enc.west) -- (enc.west);
    \draw[signal] (enc.east) -- (map.west);
    \draw[signal] (map.east) -- (pilot.west);
    \draw[signal] (pilot.east) -- (pulse.west);
    \draw[signal] (pulse.east) -- ([xshift=10pt]chan.west);
    \draw[signal] ([yshift=3pt] chan.south) -- (filter.north);
    \draw[signal] (filter.west) -- (oversampling.east);
    \draw[signal] (oversampling.west) -- (sync.east);
    \draw[signal] (sync.west) -- (CSI.east);
    \draw[signal] (CSI.west) -- (dec.east);
    \draw[signal] (dec.west) -- ([xshift=-10pt]dec.west);
\end{tikzpicture}


==> diagrams/tikz_src/sync_block_backup.tex <==
% High-level view of the common-delay synchronizer.
% Blue blocks contain trainable parameters; gray blocks are fixed.
\begin{tikzpicture}[
  x=.95cm,
  y=.82cm,
  font=\scriptsize,
  text=black!85,
  >=latex,
  signal/.style={->,draw=black!65,line width=.65pt},
  wire/.style={draw=black!65,line width=.65pt},
  module/.style={
    rectangle,
    rounded corners=3pt,
    line width=.65pt,
    align=center,
    inner xsep=3pt,
    inner ysep=3pt,
    minimum height=.80cm
  },
  learned/.style={module,draw=e2eBlue,fill=e2eBlueFill},
  fixed/.style={module,draw=black!42,fill=black!4},
  edgelabel/.style={fill=white,inner xsep=2pt,inner ysep=1pt},
  junction/.style={circle,fill=black!65,inner sep=0pt,minimum size=2.3pt}
]

\node[font=\footnotesize] (input) at (0,2.00) {$\matY$};

\node[fixed,text width=2.25cm] (cues) at (1.95,2.75)
  {\textbf{\footnotesize Candidate cues}\\[-1pt]
   window/boundary power\\[-1pt]
   adjacent correlation};

\node[learned,text width=2.15cm] (heads) at (4.70,2.75)
  {\textbf{\footnotesize Candidate heads}\\[-1pt]
   $p_q$ and fractional corrections};

\node[learned,text width=2.40cm] (context) at (3.30,1.18)
  {\textbf{\footnotesize Temporal context}\\[-1pt]
   full complex packet};

\node[fixed,text width=2.00cm] (fusion) at (7.05,2.00)
  {\textbf{\footnotesize Refine + soft fuse}\\[-1pt]
   $\sum_q p_q(qt_s+\hat e_q)$};

\node[fixed,text width=2.75cm] (correction) at (5.50,0)
  {\textbf{\footnotesize Pulse-model correction}\\[-1pt]
   symbol-wise LMMSE};

\node[font=\footnotesize] (output) at (8.05,0) {$\matY'$};

\coordinate (split) at (.48,2.00);
\draw[wire] (input.east)--(split);
\node[junction] at (split) {};
\draw[signal] (split)|-(cues.west);
\draw[signal] (split)|-(context.west);

\draw[signal] (cues.east)--(heads.west);
\draw[signal] (heads.east)--(fusion.north west);
\draw[signal] (context.east)--(fusion.south west);

\draw[signal] (input.south)--(0,0)--(correction.west)
  node[pos=.63,above,edgelabel] {$\matY$};
\draw[signal] (fusion.south)--(7.05,.62)--(5.50,.62)--(correction.north)
  node[pos=.48,above,edgelabel] {$\hat d$};
\draw[signal] (correction.east)--(output.west);

\end{tikzpicture}

